Revisiting EZBFT: A Decentralized Byzantine Fault Tolerant Protocol with Speculation

In this note, we revisit EZBFT[2] and present safety, liveness and execution consistency violations in the protocol. To demonstrate these violations, we present simple scenarios, involving only four replicas, two clients, and one or two owner changes. We also note shortcomings of the presented TLA+ specification used to model check the proposed protocol.

==> sections/rough.tex <==

Consider four replicas $i_1$, $i_2$, $i_3$, $i_4$ of which one, $i_1$, is byzantine and three clients $c_1$, $c_2$ and $c_3$ of which $c_1$ is byzantine.

\begin{itemize}[]
\item \textbf{Client $c_1$ proposing request $a$ and Client $c_2$ proposing request $b$ such that requests $a$ and $b$ interfere}

\begin{enumerate}[1.]
    \item Client $c_1$ sends its request $a$ to replica $i_1$ which is byzantine. Replica $i_1$ assigns empty dependencies and sequence number of 1 to request $a$. Replica $i_1$ assigns instance $i_1.0$ to $\langle a, \{\}, 1 \rangle$.
    \item At the same time, client $c_2$ sends its request $b$ to replica $i_2$.  Replica $i_2$ assigns empty dependencies and sequence number of 1 to request $b$. Replica $i_2$ assigns instance $i_2.0$ to $\langle b, \{\}, 1 \rangle$.
    \item Replica $i_1$ sends SPEC-ORDER messages to all replicas for $\langle a, \{\}, 1 \rangle$ at instance $i_1.0$.
    \item Replica $i_2$ sends SPEC-ORDER messages to all replicas for $\langle b, \{\}, 1 \rangle$ at instance $i_2.0$.
    \item Replica $i_2$ updates dependency and sequence number for request $a$ to be $\langle a, \{b\}, 2 \rangle$ and responds to client $c_1$ in SPEC-REPLY of the form $\langle a, \{b\}, 2 \rangle$.
    \item Replica $i_1$, $i_2$ and $i_4$ sends $\langle a, \{\}, 1 \rangle$ to client $c_1$ in SPEC-REPLY.
    \item Replica $i_1$ receives SPEC-ORDER message with $\langle b, \{\}, 1 \rangle$ from replica $i_2$.
    \item Client $c_1$ collects all $3f+1$ SPEC-REPLY responses. Three responses have form $\langle a, \{\}, 1 \rangle$ while one has form $\langle a, \{b\}, 2 \rangle$.
    \item Client $c_1$ equivocates and forms two \textit{commit certificate}. One \textit{commit certificate} with $2f+1$ identical responses of the form $\langle a, \{\}, 1 \rangle$. Call this \textit{commit certificate} $CC1$.  Another \textit{commit certificate} contains $f+1$ responses of the form $\langle a, \{\}, 1 \rangle$ and $f$ responses of the form $\langle a, \{b\}, 2 \rangle$. Call this \textit{commit certificate} $CC2$.
    \item Client $c_1$ sends $CC1$ to replicas $i_1$, $i_3$ and $i_4$ and $CC2$ to replica $i_2$.
    \item Client $c_1$ collects identical $2f+1$ COMMIT-REPLY from replica $i_1$, $i_3$ and $i_4$ and considers $\langle a, \{\}, 1 \rangle$ \textit{committed}.
\end{enumerate}

\item \textbf{Client $c_3$ proposing request $c$ which interferes with requests $a$ and $b$.}
\begin{enumerate}[1.]
\item Client $c_3$ sends its request $c$ to replica $i_3$.
\item Replica $i_3$ assigns empty dependencies and sequence number of 1 to request $c$. Replica $i_3$ assigns instance $i_3.0$ to $\langle c, \{a\}, 2 \rangle$.
\item Replica $i_3$ sends SPEC-ORDER messages to all replicas for command $\langle c, \{a\}, 2 \rangle$.
\item Replica $i_1$ equivocates and recomputes its history based on the execution of request $\langle a, \{b\}, 2 \rangle$.  Replica $i_1$ speculatively executes request $\langle c, \{a\}, 3 \rangle$ and sends SPEC-REPLY to client $c_3$.
\item Replica $i_2$ received $CC2$ for request $\langle a, \{b\}, 2 \rangle$. Its execution history is bound to be similar to H2 with a \textit{commit certificate} $CC2$
\item Replica $i_3$ received $CC1$. Its execution history will based on execution of $\langle a, \{\}, 1 \rangle$. Call this history H1.
\item Client $c_3$ receives $2f+1$ SPEC-REPLY with unequal execution histories. 
 \begin{itemize}
     \item Replica $i_1$ sends history H2 for request $\langle a, \{b\}, 2 \rangle$.
     \item Replica $i_2$ sends history H2 for request $\langle a, \{b\}, 2 \rangle$ with a commit certificate $CC2$
     \item Replica $i_3$ sends history H1 for request $\langle a, \{\}, 1\rangle$ with a commit certificate $CC1$.
 \end{itemize}

At this stage of protocol execution, there are no specification for how client $c_3$ should resolve the situation. However, it seems likely to choose command  
 $\langle a, \{b\}, 2 \rangle$ as it contains $f+1$ SPEC-REPLY from replicas $i_1$ and $i_2$ with a commit certificate $CC2$. However, if command $\langle a, \{b\}, 2 \rangle$ is chosen, it would violate safety.
\end{enumerate}
\end{itemize}
